Towards Real-time Text-driven Image Manipulation with Unconditional Diffusion Models

Recent advances in diffusion models enable many powerful instruments for image editing. One of these instruments is text-driven image manipulations: editing semantic attributes of an image according to the provided text description. % Popular text-conditional diffusion models offer various high-quality image manipulation methods for a broad range of text prompts. Existing diffusion-based methods already achieve high-quality image manipulations for a broad range of text prompts. However, in practice, these methods require high computation costs even with a high-end GPU. This greatly limits potential real-world applications of diffusion-based image editing, especially when running on user devices. In this paper, we address efficiency of the recent text-driven editing methods based on unconditional diffusion models and develop a novel algorithm that learns image manipulations 4.5-10 times faster and applies them 8 times faster. We carefully evaluate the visual quality and expressiveness of our approach on multiple datasets using human annotators. Our experiments demonstrate that our algorithm achieves the quality of much more expensive methods. Finally, we show that our approach can adapt the pretrained model to the user-specified image and text description on the fly just for 4 seconds. In this setting, we notice that more compact unconditional diffusion models can be considered as a rational alternative to the popular text-conditional counterparts.

==> limitations.tex <==
\section{Limitations and future work}
\dmitry{just a rough draft. Needs to be elaborated and properly reformulated. We can remove this sect later on if everyone votes for this.}

1) Both methods (DiffusionCLIP and ours) require exhausting hyperparameter search.

2) There are no automated metrics for the editing quality assessment.

3) Inconsistent results (poor generalization): it works almost perfectly on some images but can completely fail on many others.

4) Fine-tune the entire diffusion model is cumbersome, we can do it easier for sure.

5) smth else
